Framework to coordinate ubiquitous devices with SOA standards

Context: Ubiquitous devices and pervasive environments are in permanent interaction in people's daily lives. In today's hyper-connected environments, it is necessary for these devices to interact with each other, transparently to the users. The problem is analyzed from the different perspectives that compose it: SOA, service composition, interaction, and the capabilities of ubiquitous devices. Problem: Currently, ubiquitous devices can interact in a limited way due to the proprietary mechanisms and protocols available on the market. The few proposals from academia have hardly achieved an impact in practice. This is not in harmony with the situation of the Internet environment and web services, which have standardized mechanisms for service composition. Aim: Apply the principles of SOA, currently standardized and tested in the information systems industry, for the connectivity of ubiquitous devices in pervasive environments. For this, a coordination framework based on these technologies is proposed. Methodology: We apply an adaptation of Design Science in our environment to allow the iterative construction and evaluation of prototypes. For this, a proof of concept is developed on which this methodology and its cycles are based. Results: We built and put into operation a coordination framework for ubiquitous devices based on WS-CDL, along with a proof of concept. In addition, we contribute to the WS-CDL language in order to support the characteristics of specific ubiquitous devices.

==> Imagenes/metodologia <==
{"contentType":"application/gliffy+json","version":"1.1","metadata":{"title":"untitled","revision":0,"exportBorder":false},"embeddedResources":{"index":0,"resources":[]},"stage":{"objects":[{"x":649.4318181818182,"y":148.31578947368422,"rotation":0,"id":58,"uid":"com.gliffy.shape.uml.uml_v1.default.message","width":96.59090909090908,"height":94.73684210526316,"lockAspectRatio":false,"lockShape":false,"order":26,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":2,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":false,"interpolationType":"linear","cornerRadius":0,"controlPath":[[-1.9318181818182438,3.7894736842105203],[14.488636363636488,101.36842105263162]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":15,"px":0.5,"py":1}}},"linkMap":[]},{"x":167.3165052160954,"y":153.02279320348117,"rotation":0,"id":53,"uid":"com.gliffy.shape.uml.uml_v1.default.message","width":93.4239940387481,"height":91.7530045586407,"lockAspectRatio":false,"lockShape":false,"order":25,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":2,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":false,"interpolationType":"linear","cornerRadius":0,"controlPath":[[74.5016766020864,-0.9175300455864317],[479.2175856929957,90.02983837546623]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":12,"px":0.5,"py":1}}},"linkMap":[]},{"x":143.96050670640832,"y":147.51761292996275,"rotation":0,"id":52,"uid":"com.gliffy.shape.uml.uml_v1.default.message","width":93.4239940387481,"height":91.7530045586407,"lockAspectRatio":false,"lockShape":false,"order":24,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":2,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":false,"interpolationType":"linear","cornerRadius":0,"controlPath":[[97.85767511177349,4.587650227931988],[279.33774217585665,117.44384583506013]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":12,"px":0.5,"py":1}}},"linkMap":[]},{"x":639.7727272727274,"y":138.84210526315792,"rotation":0,"id":31,"uid":"com.gliffy.shape.uml.uml_v1.default.message","width":96.59090909090908,"height":94.73684210526316,"lockAspectRatio":false,"lockShape":false,"order":23,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":2,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":false,"interpolationType":"linear","cornerRadius":0,"controlPath":[[7.727272727272634,13.263157894736821],[-176.76136363636363,114.63157894736844]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":15,"px":0.5,"py":1}}},"linkMap":[]},{"x":504.54545454545456,"y":138.84210526315792,"rotation":0,"id":30,"uid":"com.gliffy.shape.uml.uml_v1.default.message","width":96.59090909090908,"height":94.73684210526316,"lockAspectRatio":false,"lockShape":false,"order":22,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":2,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":false,"interpolationType":"linear","cornerRadius":0,"controlPath":[[7.727272727272691,13.263157894736821],[124.60227272727269,116.52631578947373]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":14,"px":0.5,"py":1}}},"linkMap":[]},{"x":366.42045454545456,"y":141.68421052631578,"rotation":0,"id":29,"uid":"com.gliffy.shape.uml.uml_v1.default.message","width":96.59090909090908,"height":94.73684210526316,"lockAspectRatio":false,"lockShape":false,"order":21,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":2,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":false,"interpolationType":"linear","cornerRadius":0,"controlPath":[[15.454545454545439,10.42105263157896],[67.61363636363632,110.84210526315789]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":13,"px":0.5,"py":1}}},"linkMap":[]},{"x":126.20994783904621,"y":146.60008288437632,"rotation":0,"id":27,"uid":"com.gliffy.shape.uml.uml_v1.default.message","width":93.4239940387481,"height":91.7530045586407,"lockAspectRatio":false,"lockShape":false,"order":20,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":2,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":false,"interpolationType":"linear","cornerRadius":0,"controlPath":[[115.6082339791356,5.50518027351842],[82.76732488822651,101.1893907998342]],"lockSegments":{}}},"children":null,"constraints":{"constraints":[],"startConstraint":{"type":"StartPositionConstraint","StartPositionConstraint":{"nodeId":12,"px":0.5,"py":1}}},"linkMap":[]},{"x":734.4318181818181,"y":38.421052631578945,"rotation":0,"id":16,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.process","width":100.00000000000011,"height":113.68421052631581,"lockAspectRatio":false,"lockShape":false,"order":18,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#EEEEEE","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.500000000000003,"y":0,"rotation":0,"id":23,"uid":null,"width":95.00000000000011,"height":16,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 14px; font-family: Arial; white-space: pre-wrap; line-height: 16.5px; color: rgb(0, 0, 0);\">Comunicación</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":599.2045454545455,"y":38.421052631578945,"rotation":0,"id":15,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.process","width":96.59090909090908,"height":113.68421052631581,"lockAspectRatio":false,"lockShape":false,"order":16,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#EEEEEE","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.4147727272727275,"y":0,"rotation":0,"id":22,"uid":null,"width":91.76136363636364,"height":16,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 14px; font-family: Arial; white-space: pre-wrap; line-height: 16.5px; color: rgb(0, 0, 0);\">Evaluación</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":463.9772727272727,"y":38.421052631578945,"rotation":0,"id":14,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.process","width":96.59090909090908,"height":113.68421052631581,"lockAspectRatio":false,"lockShape":false,"order":14,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#EEEEEE","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.4147727272727275,"y":0,"rotation":0,"id":21,"uid":null,"width":91.76136363636364,"height":16,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 14px; font-family: Arial; white-space: pre-wrap; line-height: 16.5px; color: rgb(0, 0, 0);\">Demostración</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":328.75,"y":38.421052631578945,"rotation":0,"id":13,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.process","width":106.25000000000001,"height":113.68421052631581,"lockAspectRatio":false,"lockShape":false,"order":12,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#EEEEEE","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.65625,"y":0,"rotation":0,"id":20,"uid":null,"width":100.93750000000001,"height":48,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 14px; font-family: Arial; white-space: pre-wrap; line-height: 16.5px; color: rgb(0, 0, 0);\">Diseño y desarrollo del artefacto</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":193.52272727272728,"y":38.421052631578945,"rotation":0,"id":12,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.process","width":96.59090909090908,"height":113.68421052631581,"lockAspectRatio":false,"lockShape":false,"order":10,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#EEEEEE","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.146464646464647,"y":0,"rotation":0,"id":19,"uid":null,"width":92.29797979797979,"height":32,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 14px; font-family: Arial; white-space: pre-wrap; line-height: 16.5px; color: rgb(0, 0, 0);\">Definición de los objeteivos</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":58.29545454545454,"y":38.421052631578945,"rotation":0,"id":10,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.process","width":96.59090909090908,"height":113.68421052631581,"lockAspectRatio":false,"lockShape":false,"order":8,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#EEEEEE","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.4147727272727275,"y":0,"rotation":0,"id":18,"uid":null,"width":91.76136363636364,"height":32,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 14px; font-family: Arial; white-space: pre-wrap; line-height: 16.5px; color: rgb(0, 0, 0);\">Identificación del problema</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":-111.70454545454544,"y":94.31578947368422,"rotation":0,"id":25,"uid":"com.gliffy.shape.uml.uml_v1.default.association","width":96.59090909090908,"height":94.73684210526316,"lockAspectRatio":false,"lockShape":false,"order":7,"graphic":{"type":"Line","Line":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"none","dashStyle":null,"startArrow":0,"endArrow":0,"startArrowRotation":"auto","endArrowRotation":"auto","ortho":true,"interpolationType":"linear","cornerRadius":0,"controlPath":[[132.32954545454544,0.9473684210526316],[547.6704545454546,0.9473684210526316],[547.6704545454546,0.9473684210526316],[963.0113636363635,0.9473684210526316]],"lockSegments":{}}},"children":[],"linkMap":[]},{"x":10,"y":10,"rotation":0,"id":5,"uid":"com.gliffy.shape.flowchart.flowchart_v1.default.process","width":850,"height":180,"lockAspectRatio":false,"lockShape":false,"order":6,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.rectangle.basic_v1","strokeWidth":2,"strokeColor":"#333333","fillColor":"#EEEEEE","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[],"linkMap":[]},{"x":578.5018939393939,"y":227.89473684210523,"rotation":0,"id":42,"uid":"com.gliffy.shape.basic.basic_v1.default.ellipse","width":155.92992424242428,"height":142.10526315789474,"lockAspectRatio":false,"lockShape":false,"order":4,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.ellipse.basic_v1","strokeWidth":2,"strokeColor":"#666666","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.0790656565656565,"y":0,"rotation":0,"id":43,"uid":null,"width":151.77179292929296,"height":90,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 13px; font-family: Arial; white-space: pre-wrap; line-height: 15.5px; color: rgb(0, 0, 0);\">PI3\n</span></p><p style=\"text-align:center;\"><span style=\"font-size: 13px; font-family: Arial; white-space: pre-wrap; line-height: 15.5px; color: rgb(0, 0, 0);\">¿Es posible demostrar la aplicabilidad de SOA en ambientes ubicuos mediante una prueba de concepto?</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":356.97064393939394,"y":227.89473684210523,"rotation":0,"id":40,"uid":"com.gliffy.shape.basic.basic_v1.default.ellipse","width":156.05871212121204,"height":142.10526315789474,"lockAspectRatio":false,"lockShape":false,"order":2,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.ellipse.basic_v1","strokeWidth":2,"strokeColor":"#666666","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.0807828282828265,"y":0,"rotation":0,"id":41,"uid":null,"width":151.89714646464637,"height":75,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 13px; font-family: Arial; white-space: pre-wrap; line-height: 15.5px; color: rgb(0, 0, 0);\">PI2\n</span></p><p style=\"text-align:center;\"><span style=\"font-size: 13px; font-family: Arial; white-space: pre-wrap; line-height: 15.5px; color: rgb(0, 0, 0);\">¿Es posible desarrollar un framework que permita incorporar SOA a dispositivos ubicuos?</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]},{"x":133.92613636363643,"y":227.89473684210523,"rotation":0,"id":38,"uid":"com.gliffy.shape.basic.basic_v1.default.ellipse","width":156.18749999999986,"height":142.10526315789474,"lockAspectRatio":false,"lockShape":false,"order":0,"graphic":{"type":"Shape","Shape":{"tid":"com.gliffy.stencil.ellipse.basic_v1","strokeWidth":2,"strokeColor":"#666666","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"state":0,"shadowX":0,"shadowY":0,"opacity":1}},"children":[{"x":2.0824999999999982,"y":0,"rotation":0,"id":39,"uid":null,"width":152.02249999999987,"height":75,"lockAspectRatio":false,"lockShape":false,"order":"auto","graphic":{"type":"Text","Text":{"tid":null,"valign":"middle","overflow":"none","vposition":"none","hposition":"none","html":"<p style=\"text-align:center;\"><span style=\"font-size: 13px; font-family: Arial; white-space: pre-wrap; line-height: 15.5px; color: rgb(0, 0, 0);\">PI1\n</span></p><p style=\"text-align:center;\"><span style=\"font-size: 13px; font-family: Arial; white-space: pre-wrap; line-height: 15.5px; color: rgb(0, 0, 0);\">Es SOA capaz de actuar como mecanismo de coordinación de sistemas ubicuos?</span></p>","paddingLeft":2,"paddingRight":2,"paddingBottom":2,"paddingTop":2}},"children":null}],"linkMap":[]}],"background":"#FFFFFF","width":860,"height":370,"maxWidth":5000,"maxHeight":5000,"nodeIndex":60,"autoFit":true,"exportBorder":false,"gridOn":true,"snapToGrid":true,"drawingGuidesOn":true,"pageBreaksOn":false,"printGridOn":false,"printPaper":"LETTER","printShrinkToFit":false,"printPortrait":true,"shapeStyles":{"com.gliffy.shape.flowchart.flowchart_v1.default":{"fill":"#FFFFFF","stroke":"#333333","strokeWidth":2},"com.gliffy.shape.flowchart.flowchart_v2.default":{"fill":"#FFFFFF","stroke":"#3399FF","strokeWidth":2,"gradient":true}},"lineStyles":{},"textStyles":{},"themeData":{"uid":"com.gliffy.theme.daily_glyph","name":"The Daily Glyph","shape":{"primary":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"#EEEEEE","gradient":false,"dropShadow":false,"opacity":1,"text":{"color":"#000000","bold":null,"italic":null,"underline":null}},"secondary":{"strokeWidth":2,"strokeColor":"#666666","fillColor":"#FFFFFF","gradient":false,"dropShadow":false,"opacity":1,"text":{"color":"#000000","bold":null,"italic":null,"underline":null}},"tertiary":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"#CCCCCC","gradient":false,"dropShadow":false,"opacity":1,"text":{"color":"#000000","bold":null,"italic":null,"underline":null}},"highlight":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"#333333","gradient":false,"dropShadow":false,"opacity":1,"text":{"color":"#FFFFFF","bold":null,"italic":null,"underline":null}}},"line":{"strokeWidth":2,"strokeColor":"#333333","fillColor":"none","arrowType":2,"interpolationType":"linear","cornerRadius":0,"text":{"color":"#000000","bold":null,"italic":null,"underline":null}},"text":{"color":"#000000","bold":null,"italic":null,"underline":null},"stage":{"color":null}}}}
